Putting People in LLMs' Shoes: Generating Better Answers via Question Rewriter

Large Language Models (LLMs) have demonstrated significant capabilities, particularly in the domain of question answering (QA). However, their effectiveness in QA is often undermined by the vagueness of user questions. To address this issue, we introduce single-round instance-level prompt optimization, referred to as question rewriter. By enhancing the intelligibility of human questions for black-box LLMs, our question rewriter improves the quality of generated answers. The rewriter is optimized using direct preference optimization based on feedback collected from automatic criteria for evaluating generated answers; therefore, its training does not require costly human annotations. The experiments across multiple black-box LLMs and long-form question answering (LFQA) datasets demonstrate the efficacy of our method. This paper provides a practical framework for training question rewriters and sets a precedent for future explorations in prompt optimization within LFQA tasks. Code is available at https://github.com/3244we/Question-Rewriter.

==> Ablation_Study.tex <==

\begin{table*}[htbp]
\centering
\large
\setlength{\tabcolsep}{3pt} % Reduce the space between columns to fit the table better
\renewcommand{\arraystretch}{1}
\begin{tabular}{@{}lrrrrrr@{}} % Ensure the number of columns here matches the content
\toprule
\textbf{Metric} & \textbf{Method} & \textbf{Original} & \textbf{Best-Random} & \textbf{Random-Worst} & \textbf{Best-Worst} & \textbf{Random-Random} \\
\midrule
\multirow{6}{*}{\bm{$S_\textbf{comp} \uparrow$}} & Llama-3-8B       & 0.4573 & \textbf{0.4600} & 0.4276          & 0.4026          & 0.4564 \\
                                                  & Mistral-7B-v0.2 & 0.4374 & \textbf{0.4899} & \textbf{0.4643} & 0.4304          & \textbf{0.4746} \\
                                                  & Zephyr-7B-beta  & 0.4396 & \textbf{0.4702} & \textbf{0.4607} & \textbf{0.4586} & \textbf{0.4650} \\
                                                  & Gemma-1.1-7B    & 0.4010 & \textbf{0.4956} & \textbf{0.4304} & \textbf{0.4065} & \textbf{0.4655} \\
                                                  & GPT-3.5-turbo   & 0.4909 & \textbf{0.4978} &     0.4905      & 0.4598          & \textbf{0.5302} \\
                                                  & GPT-4o          & 0.5167 & \textbf{0.6253} & \textbf{0.5759} & \textbf{0.5382} & \textbf{0.5520} \\
\midrule
\multirow{6}{*}{\bm{$S_\textbf{cont}\downarrow$}} & Llama-3-8B      & 0.4400 & \textbf{0.4000} & \textbf{0.4000} & \textbf{0.4000} & \textbf{0.4000} \\
                                                  & Mistral-7B-v0.2 & 0.2200 & 0.2600          & 0.2200          & 0.2400          & 0.3400 \\
                                                  & Zephyr-7B-beta  & 0.3400 & \textbf{0.2600} & \textbf{0.2800} & \textbf{0.3000} & \textbf{0.2600} \\
                                                  & Gemma-1.1-7B    & 0.5400 & \textbf{0.2200} & \textbf{0.3800} & \textbf{0.4000} & \textbf{0.3400} \\
                                                  & GPT-3.5-turbo   & 0.3200 & \textbf{0.2800} & \textbf{0.3000} & \textbf{0.3000} & \textbf{0.2600} \\
                                                  & GPT-4o          & 0.2800 & \textbf{0.2400} & \textbf{0.2000} & \textbf{0.2200} & 0.3200 \\
\bottomrule
\end{tabular}
\caption{Ablation study of the different sampling combination for $\mathcal{P}(q)$. \textbf{Bold} indicates the rewriter trained by the $\mathcal{P}(q)$ sampled by this combination performing better than the corresponding original for this LLM.}
\label{tab:sample_methods}
\end{table*}

\section{Comparison for Sampling Combination}

We test the performance of rewriters trained by $\mathcal{P}(q)$ sampled by different sampling combination on the K-QA dataset. There are four sampling combinations in total, where $\mathcal{Q}_+$ can be either the top $N_+$ questions or randomly sampled, and $\mathcal{Q}_-$ can be either the bottom $N_-$ questions or randomly sampled. Table \ref{tab:sample_methods} shows that rewriters trained by the Best-Random combination, which is the combination we currently use, perform the best, failing to optimize only one metric in one model. The Random-Random combination is effective across most models and metrics. The other three compositions all have 3 or 4 metrics worse than the corresponding original.



